Deep Momentum Multi-Marginal Schr\"odinger Bridge

It is a crucial challenge to reconstruct population dynamics using unlabeled samples from distributions at coarse time intervals. Recent approaches such as flow-based models or Schr\"odinger Bridge (SB) models have demonstrated appealing performance, yet the inferred sample trajectories either fail to account for the underlying stochasticity or are $\underline{D}$eep $\underline{M}$omentum Multi-Marginal $\underline{S}$chr\"odinger $\underline{B}$ridge(DMSB), a novel computational framework that learns the smooth measure-valued spline for stochastic systems that satisfy position marginal constraints across time. By tailoring the celebrated Bregman Iteration and extending the Iteration Proportional Fitting to phase space, we manage to handle high-dimensional multi-marginal trajectory inference tasks efficiently. Our algorithm outperforms baselines significantly, as evidenced by experiments for synthetic datasets and a real-world single-cell RNA sequence dataset. Additionally, the proposed approach can reasonably reconstruct the evolution of velocity distribution, from position snapshots only, when there is a ground truth velocity that is nevertheless inaccessible.

==> subtex/intro2.tex <==
\section{Introduction}
\textbf{Score-based Generative Model (SGM)} \cite{song2020score} is an emerging class of generative models that have exhibited remarkable success in image generation, editing, and translation \cite{dhariwal2021diffusion,meng2021sdedit,saharia2022palette}. Similar to many other generative models, SGM aims to identify nonlinear maps that convert simple prior distributions, typically Gaussian, into complex and often intractable data distributions. SGM accomplishes this task by first diffusing data to noise through a pre-specified stochastic differential equation (SDE), followed by learning to reverse this diffusion process by performing regression on a network to obtain the score function at each time step. This reversal of the diffusion process consequently establishes the generation.The Critically-damped Langevin Diffusion (CLD) \cite{dockhorn2021score} extends the pre-defined SDE into the phase space by introducing an auxiliary velocity variable with a tractable Gaussian distribution at both the initial and terminal time. The resulting trajectory in the position space becomes smoother, as stochasticity is only injected into the velocity space, and the empirical performance and sample efficiency are enhanced due to the structure of the critical damped SDE. However, SGM faces several constraints. Firstly, the diffusion process must adhere to a simple form to compute the analytic score function for the regression process. Secondly, the diffusion process must run for a sufficient amount of time steps to approximate the end distribution of position as Gaussian. Thirdly, the prior distribution must be Gaussian. \guan{there're a few non-Gaussian prior SGM models like cold diffusions.} In addition, CLD sets both boundary velocity distributions to be Gaussian. 

\textbf{Schr\"odinger Bridge (SB)} is an entropy regularized optimal transport that provides an alternative perspective for constructing the SDE process, offering a solution to the limitations of SGM. SB seeks the \emph{straightest} path measure between two \emph{arbitrary} distributions by minimizing transportation cost (i.e. 2-Wasserstein distance ($W_2$)) regularized by an additional entropic term. While SB mitigates the issues presented in SGM, solving high-dimensional SB problem is challenging. Recent work \cite{chen2021likelihood,de2021diffusion} have elaborated the connection between SGM and SB, and proposed the scalable mean matching Iterative Proportional Fitting algorithm (IPF) to estimate SB. Applications of SB, such as image-to-image transformation and RNA trajectory inference \cite{koshizuka2022neural,liu20232}, demonstrate the effectiveness of SB in various domains.

\tao{honestly i feel it should be SGM vs SB, instead of SGM vs SB, because SB is still based on diffusion process. i'm also unsure whether we should oppose ourselves against SGM which is hot nowadays}

\tao{in any case, shall we mention that for SB, both marginals can be arbitrary, but for `SGM', one of them is usually Gaussian?}

\textbf{Trajectory Inference:} Understanding the population dynamics of time-evolving individuals received considerable attention recently. The associating applications appear in various scientific areas such as estimating cell dynamics \cite{schiebinger2019optimal,yang2018scalable}, predicting meteorological evolution \cite{fisher2009data} and medical healthcare statistics tracking \cite{manton2008cohort}. Central to research along this line is to understand the dynamics and reactions of individuals given static snapshot samples taken at sporadic time points. \cite{hashimoto2016learning,bunne2022proximal} constructed an energy landscape that best aligned with empirical observations using neural network. \cite{tong2020trajectorynet,huguet2022manifold} learn regularized Neural ODE \cite{chen2018neural} to encode such potential landscape. Notably, in the aforementioned work, the trajectory of samples is represented in a deterministic way. In contrast, \cite{koshizuka2022neural,chizat2022trajectory} employ SB to determine the most likely evolution of samples between marginal distributions when individual sample trajectories are also affected by environmental stochasticity. Yet, these approaches scale poorly w.r.t. the state dimension due to specialized neural network architectures and computational frameworks.

\begin{table}[H]
    \caption{Summary of the differences between SGM, CLD, SB and our DMSB.}\label{table:diff_summary}
    \begin{center}
        \begin{tabular}{ccccc}
            \toprule
            models & Optimality& Boundary Positions& Boundary Velocities\\[1pt]
            \hline
            SGM \cite{song2020score} & \xmark & Gaussian,data\\[1pt]
            CLD \cite{dockhorn2021score} & \xmark & Gaussian,data&Gaussians\\[1pt]
            \bottomrule
            SB \cite{chen2021likelihood} & $\downarrow W_2\rightarrow$ kinks & Arbitrary,Arbitrary&-\\[1pt]
            DMSB (ours)  & $\downarrow W_2\rightarrow$ smooth& Arbitrary,Arbitrary&Learned\\[1pt]
            \bottomrule
        \end{tabular}
    \end{center}
\end{table}

\guan{ Maybe try this
\begin{table}[H]
    \caption{Comparison between different models in terms of optimality and boundary distributions $p_0$ and $p_1$. Our DMSB extends standard SB, which generalizes SGM beyond Gaussian priors, to phase space, similar to CLD. However, unlike CLD, DMSB jointly \emph{learns} the phase space distributions, i.e., $p_{\theta}(x,v) = p_\calA(x) q_\theta(v|x)$ and $p_{\phi}(x,v) = p_\calB(x) q_\phi(v|x)$. In other words, DMSB infers the underlying phase state dynamics given only state distributions.
    \guan{Add explanation for optimality}
    }
    \begin{center}
        \begin{tabular}{ccccc}
            \toprule
            models & Optimality& $p_0(\cdot)$ & $p_1(\cdot)$ \\[1pt]
            \hline
            SGM \cite{song2020score} & \xmark & $p_\calA(x)$ & $\calN(0,1)$ \\[1pt]
            CLD \cite{dockhorn2021score} & \xmark & $p_\calA(x) \otimes \calN(0,1) $ &  $\calN(0,1) \otimes \calN(0,1)$ \\[1pt]
            % \bottomrule
            SB \cite{chen2021likelihood} & $\downarrow W_2\rightarrow$ kinks & $p_\calA(x)$ & $p_\calB(x)$ \\[1pt]
            DMSB (ours)  & $\downarrow W_2\rightarrow$ smooth& $p_\calA(x) q_\theta(v|x) $ & $p_\calB(x) q_\phi(v|x)$\\[1pt]
            \bottomrule
        \end{tabular}
    \end{center}
\end{table}
}

In this work, we start with SB in phase space (termed  momentum SB, mSB), and then further investigate mSB with multiple empirical marginal constraints present in the position space, which was formulated as multi-marginal mSB (mmmSB) in \cite{chen2019multi} \tao{need to specify what's different from chen2019multi}. The optimality of transportation cost in SB leads to straight trajectories, and if one solves N-1 SB problems and connect the resulting trajectories to match N marginals, the connected trajectories will have kinks at all connection points. On the contrary, in mmmSB, the optimality of transportation cost leads to a smooth measure-spline over the state space that also interpolates the empirical marginals. This approach is highly suitable for addressing the challenge of trajectory inference in single-cell RNA sequencing, and our research will place a specific emphasis on solving mmmSB in high-dimensional cases and exploring this application in subsequent sections.  The main contributions of our work are fourfold:
\begin{itemize}[leftmargin=0.5cm]
    \item We extend the mean matching IPF to phase space allowing for scalable mSB computing.
    \item We introduce and tailor the Bregman Iteration \cite{bregman1967relaxation} for mmmSB which makes it compatible with the phase space mean matching objective, thus the efficient computation is activated for high dimensional momentum multi-marginal SB. 
    \item We show how to overcome the challenge of sampling the velocity variable when it is not available in training data, which enhances the applicability of our model.
    \item We show the performance of proposed algorithm DMSB on toy datasets which contains intricate bifurcations and merge. On realistic high-dimension (100-D) single-cell RNA-seq (scRNA-seq) datasets, DMSB outperforms baselines by a significant margin in terms of the quality of the generated trajectory both visually and quantitatively. We show that DMSB is able to capture reasonable velocity distribution compared with ground truth while other baselines fail.
\end{itemize}



==> subtex/mmmSB2.tex <==
\begin{figure}[t]
  \includegraphics[width=\textwidth]{fig/semicircle_SB_together.pdf}
  \caption{The problem definitions of different SB problems and corresponding algorithms. The toy example presented below indicates that an SB problem endeavors to determine the most direct path between empirical marginals that contain additive noise, while a multi-marginal momentum SB problem endeavors to establish a smooth measure-spline between marginals in the position space.}
  \label{fig:diff-approach}
\end{figure}
\section{Momentum Schr\"odinger Bridge}\label{sec:mmmSB}
We first introduce half-bridge IPF training in the phase space which can be used to solve momentum SB (mSB) problem with two marginals constraints. This scalable phase space half-bridge technique can be further applied to multi-marginal cases. Fig.\ref{fig:diff-approach} demonstrates how we develop an algorithm based on \cite{chen2021likelihood}. Notations used in following sections are listed in Table.\ref*{table:notation}.
\begin{table}[H]
  \begin{center}
  \begin{tabular}{cc}
    \toprule
    Notation & Definition \\[1pt]
    \hline
    $\rvx$ & position variable \\[1pt]
    $\rvv$ & velocity variable\\[1pt]
    $\rvm$ & concatenation of $\left[\rvx,\rvv\right]^\T$\\[1pt]
    \bottomrule
    \end{tabular}
    \quad
    \begin{tabular}{cc}
    \toprule
      Notation & Definition \\[1pt]
    \hline
    $\rho$ & position distribution $\rho(\rvx)$\\ [1pt]
    $\gamma$ &velocity Distribution $\gamma(\rvv)$\\[1pt]
    $\mu$    & distribution of $\mu(\rvx,\rvv)$\\ [1pt]
    \bottomrule
    \end{tabular}
  \end{center}
  \caption{Mathematical notation.}
  \label{table:notation}
\end{table}
% \vspace{-0.2in}
% \begin{table}[H]
%   \caption{Mathematical notation.}
%   \label{table:notation}
%   \vskip 0.1in
%   \begin{center}
%   \begin{small}
%   \begin{tabular}{r|cr}
%   \toprule
%   \textsc{Notation} & \textsc{Definitions}  \\
%   \midrule
%   $\mu$    & distribution of velocity and position $\mu(\rvx,\rvv)$\\ [1pt]
%   $\rho$ & position distribution $\rho(\rvx)$\\ [1pt]
%   $\gamma$ &velocity Distribution $\gamma(\rvv)$\\[1pt]
%   $\rvx$ & position variable \\[1pt]
%   $\rvv$ & velocity variable\\[1pt]
%   $\rvm$ & concatenation of $\left[\rvx,\rvv\right]^\T$\\[1pt]
%   \bottomrule
%   \end{tabular}
%   \end{small}
%   \end{center}
%   \vskip -0.1in
% \end{table}
We first introduce the concept of mSB which extends SB problem to the phase space of position and velocity. Even though for this moment, boundary distributions depend on both x and v, the goal is still to find transport maps between two distributions that only depend on position $\rvx$, and velocity $\rvv$ is an auxiliary variable artificially introduced for obtaining smooth transport. Conceptually, as an entropy regularized optimal transport problem, SB tries to obtain the straightest path between empirical probability marginals of positions $\rvx$ with additive noise, but mSB aims at finding the smooth interpolation between empirical probability marginals of $\rvx$ \cite{benamou2019second} conditioned on boundary velocity distributions (see Fig.\ref{fig:diff-approach}). Such smooth measure-valued splines in the position space is obtained by following optimization problem in the phase space \cite{chen2019multi}:

\begin{align*}
  \min_{\pi \in \Pi(\mu_0,\mu_T)} KL(\pi|\xi) \quad s.t \quad  \pi: 
  \begin{pmatrix}
    \rd \rvx_t  \\
    \rd\rvv_t  
    \end{pmatrix} &=
                  \underbrace{
                  \begin{pmatrix}
                    \rvv_t  \\
                    \mathbf{0}
                  \end{pmatrix}}_{\vf(\rvv,t)}\rd t+
                  \underbrace{
                    \begin{pmatrix}
                    \mathbf{0}&\mathbf{0}  \\
                    \mathbf{0}&g_t \\  
                  \end{pmatrix}}_{\rvg(t)}
                  \underbrace{
                  \begin{pmatrix}
                    \mathbf{0}  \\
                    \rva_t  
                  \end{pmatrix}}_{\rvu(t)}\rd t+
                  \underbrace{
                    \begin{pmatrix}
                    \mathbf{0}&\mathbf{0}  \\
                    \mathbf{0}&g_t \\  
                  \end{pmatrix}}_{\rvg(t)}\rd \rvw_t,
\end{align*}

Similar to eq.\ref{eq:sb-pde}, one can have,
\begin{theorem}[Optimal forward SDE]\label{eq:thm:opt-forward-sde}
  The optimal $\pi$ of mSB problem is induced by
  \begin{align}
    \rvu^{*}_t :=\rmZ_t\equiv         \begin{pmatrix}
        \mathbf{0} \\  
        \rvz_t
        \end{pmatrix}
    \equiv
    \begin{pmatrix}
    \mathbf{0} \\  
    g\nabla_{\markred{\rvv}}\log \Psi_t
    \end{pmatrix}
  \end{align}
  and $\Psi$ is the solution of a coupled PDE,
  % \begin{empheq}[box=\widefbox]{align*}
    % \begin{align*}
    %   &\begin{cases}
    %     &\frac{\partial \Psi}{\partial t}=-\DD\Delta_{\rvv}\Psi-\nabla_{\rvx}\Psi^\T\rvv\\
    %     &\frac{\partial \Psihat}{\partial t}=\DD\Delta_{\rvv} \hat{\Psi}-\nabla_{\rvx}\Psihat^\T \rvv
    %   \end{cases}\\
    %   &\text{s.t} \quad \Psi\Psihat=\mu(\rvx,\rvv,0), \quad \Psi\Psihat=\mu(\rvx,\rvv,T)
    % \end{align*}
    \begin{align}
      \begin{aligned}\label{eq:Psi-PDEs}
        &\begin{cases}
          &\frac{\partial \Psi_t}{\partial t}=-\DD\Delta_{\rvv}\Psi_t-\nabla_{\rvx}\Psi^\T_t\rvv\\
          &\frac{\partial \Psihat_t}{\partial t}=\DD\Delta_{\rvv} \Psihat_t-\nabla_{\rvx}\Psihat^\T_t \rvv
        \end{cases} \quad \text{s.t} \quad \Psi_0\Psihat_0=\mu(\rvx,\rvv,0), \quad \Psi_T\Psihat_T=\mu(\rvx,\rvv,T)
      \end{aligned}
    \end{align}
   The corresponding forward process is represented as:
   \begin{align}
    \rd \rvm_t  = \left[\vf + \rvg\rmZ_t \right]\rd t +\rvg(t)\rd \rvw_t \quad s.t \quad \rvm_0\sim\mu_0 \label{eq:for_opt_sde}
   \end{align}
   \begin{proof}
    see proof in Appendix \ref{appendix:thm:opt-forward-sde}.
  \end{proof}
  % \begin{align}
  %     &\rd \rvm_t  = \left[\vf + \rvg\rvu_t^{*} \right]\rd t +\rvg(t)\rd \rvw_t
  % \end{align}
\end{theorem}

Due to the special structure of $\vg(t)$, the mSB admits a simple expression in which we only require $\nabla_{\rvv}\log \Psi_t$. Thanks to time reversibility of mSB,\footnote{
  For completeness, we note that the necessary and sufficient conditions  \citep{millet1989integration} for reversing an SDE with a diffusion $\sigma(t,X_t)$ requires all elements of 
  $\nabla\cdot (\sigma\sigma^\top p_t)$ being locally integrable functions,
  % $\sum_j \nabla_{x_j} [(\sigma\sigma^\top)^{ij}p_t]$ being locally integrable functions, 
  which is trivially satisfied for our case. 
  }one can derive a similar result for optimal reverse time SDE \cite{song2021maximum,chen2021likelihood,de2021diffusion} driven by another drift term $\zhatt$ which is presented in Appendix.\ref{Appendix:thm:opt-sde}. However, obtaining the solutions of PDEs \eqref{eq:Psi-PDEs} is not trivial. Alternatively, one might create the likelihood training objective \cite{chen2021likelihood} and optimize it repeatedly as part of IPF approach to arrive at the mSB solution.
  \begin{proposition}\label{prop:likelihood-obj}
    The half-bridge IPF in phase space
    \begin{align*}
      &\pi ^{(d+1)}:=\argmin_{\pi \in \Pi(\mu_0,\cdot)}D_{KL}(\pi ||\pi ^{(d)})   \quad \rightleftarrows \quad \pi ^{(d+2)}:=\argmin_{\pi \in \Pi(\cdot,\mu_T)}D_{KL}(\pi ||\pi ^{(d+1)})
    \end{align*}
    can be represented by phase space likelihood IPF:
    \begin{align*}
      &\rmZ_t:=\argmin_{\rvz_t}-\log p(\rvm_0,0)  \quad \rightleftarrows \quad \widehat{\rmZ}_t:=\argmin_{\widehat{\rvz}_t}-\log p(\rvm_T,T).
    \end{align*}

    \begin{align*}
        \text{where}\quad \log p(\rvm_0,0)&=\E_{\widehat{\rvm}_t}\left[\log p(\widehat{\rvm}_T,T)\right]\\
        -\int_0^{T}\E_{\widehat{\rvm}_t}&\left[\underbrace{\frac{1}{2}\norm{\zhatt+\rvz_t-g\nabla_{\rvv}\log p^{SB}}^2}_{\textbf{mean matching objective}}+\frac{1}{2}\norm{\zhatt}^2-\frac{1}{2}\norm{g\nabla_{\rvv}\log p^{SB}-\zhatt}^2\right]\rd t.\\
        \text{and $\widehat{\rvm}_t$ samples from: }& \quad \rd \widehat{\rvm}_t  = \left[\vf + \rvg\Zhat_t \right]\rd t +\rvg(t)\rd \rvw_t, \quad \widehat{\rvm}_T\sim\mu_T\numberthis{}\label{eq:rev_opt_sde}
        \end{align*}
    % Meanwhile, by maximizing the log-likelihood at time $t=0$ then $t=T$ iteratively, $(\rmZ_t,\Zhatt)$ will converge to the solution of phase space SB.
    The result for $\log(\rvm_T,T)$ can be obtained in a similar derivation.
  \end{proposition}
  \begin{proof}
    see proof in Appendix \ref{z}.
  \end{proof}
  \begin{remark}
    After optimizing $\widehat{\rmZ}_t$, the reference path measure becomes eq.\ref{eq:rev_opt_sde} which implies $\pi\in \Pi(\cdot,\mu_T)$ constraint in half-bridge IPF. A path measure $\pi$ is induced by either $\rmZ_t$ (eq.\ref{eq:for_opt_sde}) or $\Zhatt$ (eq.\ref{eq:rev_opt_sde}).   As being mentioned in Remark.\ref{remark:BI-IPF}. One half-bridge IPF step is basically one BP and one IPF is one BI. Prop.\ref{prop:likelihood-obj} provides a convenient way to perform one BP in the form of $\pi:=\argmin_{\pi \in \gK_l}D_{KL}(\pi ||\bar{\pi})$ by maximizing log-likelihood given constraint $\gK$ and reference path measure $\bar{\pi}$.

  \end{remark}
  \section{Deep Momentum Multi-Marginal Schr\"odinger Bridge}\label{sec:DMSB}
We first state the problem formulation of momentum multi-marginal Schr\"odinger Bridge (mmmSB). Different from previous two marginals case, we consider the scenario where $N+1$ probability measures $\mu_{t_i}$ are lying at time $t_i$ while velocity distributions are not necessarily accessible.
\begin{proposition}[\cite{chen2019multi}]\label{Prop:mmmSB-formulation}
  The dynamical mmmSB with multiple marginal constraints reads:
  \begin{align*}
      \min_{\pi} \mathcal{J}(\pi):=\sum_{i=0}^{N-1}KL\left(\pi_{t_i,t_{i+1}}|\xi_{t_i,t_{i+1}}\right),\numberthis \label{eq:mmSB-formulation} \quad \text{s.t} \quad 
      \pi \in \mathcal{K}:=\cap_{i=0}^{N}\mathcal{K}_{t_i}
    \end{align*}
    % \label{eq:K-constraint}
    \begin{align*}
      \text{where:}\quad \mathcal{K}_{t_0}&=\left\{{\int\pi_{t_{0}t_{1}}\rd\rvm_{t_1}=\mu_{t_0}, \int\mu_{t_0}\rd\rvv_{t_0}=\rho_{t_0}}\right\}\\
      \mathcal{K}_{t_N}&=\left\{{\int\pi_{t_{N-1},t_{N}}\rd\rvm_{t_{N-1}}=\mu_{t_N}, \int\mu_{t_N}\rd\rvv_{t_N}=\rho_{t_N}}\right\}\\
      \mathcal{K}_{t_i}&=\left\{\int\pi_{t_{i}t_{t+1}}\rd\rvm_{t_{i+1}}=\mu_{t_i},\int\pi_{t_{i-1} t_{i}}\rd\rvm_{t_{i-1}}=\mu_{t_i},\int\mu_{t_i}\rd\rvv_{t_i}=\rho_{t_i}\right\},\numberthis\label{eq:mid-constraint}
    \end{align*} 
    and $\mathcal{K}$ is the intersection of close convex set of $\mathcal{K}_{t_i}$.
\end{proposition}

The problem described in Prop.\ref{Prop:mmmSB-formulation} can be solved by classical BI algorithm integrated with Sinkhorn method \cite{chen2019multi}. However, due to the curse of dimensionality and unfavorable geometric explicit solution, the BP cannot be applied in high-dimensional and continuous state space directly. To tackles these difficulties, we parameterize the forward and backward policies by a pair of neural networks. We further decouple and resemble the constraints by which it enables the scalable likelihood IPF and avoids the geometric averaging issue under mmmSB context.
\begin{figure}[t]
  \includegraphics[width=1.0\textwidth]{fig/DMSB_procedure.pdf}
  \caption{The procedure details the BI employed in DMSB. The gray and blue blocks denoted in the diagram represent the BP step performed under $\Kbound$ constraint for forward and backward policies, respectively. The red block signifies the BP step executed under the $\Kbridge$ constraint.}\label{fig:DMSB_procedure}
  \vskip -0.05in
\end{figure}
\subsection{Parameterization}
Inspired by prior work's \cite{chen2021likelihood} success, we parameterize path measure $\pi$ by forward policy $\rvz_t^{\theta}$  or backward policy $\widehat{\rvz}_t^{\phi}$ combined with certain boundary condition. We adopt Euler–Maruyama discretization and denote the timestep as $\delta_t$. Hereafter, we only demonstrate the optimization for $\rvz^\theta_t$ given reference path measure $\bar{\pi}^{\phi}$ driven by fixed $\widehat{\rvz}^\phi_t$. The procedure can be applied in the $\zhatt^{\phi}$ and vice versa.

\subsection{Decoupling and Reassembling Constraints}
We decompose the constraint set (\ref{eq:mid-constraint}) by
% \begin{align}
% \hspace*{-0.5cm}
% \begin{aligned}\label{eq:new-K-constraints}
%     \mathcal{K}_{t_i}^{0}&=\left\{{\int\pi_{t_{i}t_{t+1}}\rd\rvm_{t_{i+1}}=\hat{\mu}_{t_i}, \int\hat{\mu}_{t_i}\rd\rvv_{t_i}=\rho_{t_i}}\right\}\\
%     \mathcal{K}_{t_i}^{1}&=\left\{{\int\pi_{t_{i-1} t_{i}}\rd\rvm_{t_{i-1}}=\mu_{t_i}, \int\mu_{t_i}\rd\rvv_{t_i}=\rho_{t_i}}\right\} \\
%     \mathcal{K}_{t_i}^{2}&=\left\{{\int\pi_{t_{i}t_{t+1}}\rd\rvm_{t_{i+1}}=\int\pi_{t_{i-1} t_{i}}\rd\rvm_{t_{i-1}}}\right\}.\\
% \end{aligned}
% \end{align}
\begin{equation}\label{eq:new-K-constraints}
  \mathcal{K}_{t_i}=\cap_{r=0}^{2}\mathcal{K}_{t_i}^{r}, \quad \text{where} \quad 
  \begin{array}{l}
    \mathcal{K}_{t_i}^{0}=\left\{{\int\pi_{t_{i}t_{t+1}}\rd\rvm_{t_{i+1}}=\hat{\mu}_{t_i}, \int\hat{\mu}_{t_i}\rd\rvv_{t_i}=\rho_{t_i}}\right\}\\
    \mathcal{K}_{t_i}^{1}=\left\{{\int\pi_{t_{i-1} t_{i}}\rd\rvm_{t_{i-1}}=\mu_{t_i}, \int\mu_{t_i}\rd\rvv_{t_i}=\rho_{t_i}}\right\} \\
    \mathcal{K}_{t_i}^{2}=\left\{{\int\pi_{t_{i}t_{t+1}}\rd\rvm_{t_{i+1}}=\int\pi_{t_{i-1} t_{i}}\rd\rvm_{t_{i-1}}}\right\}.
    \end{array}
\end{equation}
  % \begin{equation}\label{eq:new-K-constraints}
  %   \mathcal{K}_{t_i}=\cap_{r=0}^{2}\mathcal{K}_{t_i}^{r}, \quad \text{where} \quad 
  % %   &\begin{array}{l}
  % %   \mathcal{K}_{t_i}^{0}&=\left\{{\int\pi_{t_{i}t_{t+1}}\rd\rvm_{t_{i+1}}=\hat{\mu}_{t_i}, \int\hat{\mu}_{t_i}\rd\rvv_{t_i}=\rho_{t_i}}\right\}\\
  % %   \mathcal{K}_{t_i}^{1}&=\left\{{\int\pi_{t_{i-1} t_{i}}\rd\rvm_{t_{i-1}}=\mu_{t_i}, \int\mu_{t_i}\rd\rvv_{t_i}=\rho_{t_i}}\right\} \\
  % %   \mathcal{K}_{t_i}^{2}&=\left\{{\int\pi_{t_{i}t_{t+1}}\rd\rvm_{t_{i+1}}=\int\pi_{t_{i-1} t_{i}}\rd\rvm_{t_{i-1}}}\right\}.
  % %   \end{array}
  % % \end{equation}
One can notice that the $\mathcal{K}_{t_i}^0$ and $\mathcal{K}_{t_i}^1$ share similar structure as simpler boundary marginal conditions $\mathcal{K}_{t_0}$ and $\mathcal{K}_{t_N}$, hence we can get rid of the notorious geometric averaging (see \S 4 in \cite{chen2019multi}). Notably, this type of constraint provides an opportunity to utilize Proposition \ref{prop:likelihood-obj} for optimization, but the joint distribution of $\rvx$ and $\rvv$ is still absent. We classify the constraints into two categories:
  \begin{align*}
      \Kbound=\left\{\cap_{i=1}^{N-1}\mathcal{K}^{r}_{t_i}\cap \mathcal{K}_{t_0}\cap \mathcal{K}_{t_{N}}|\forall r \in \left\{0,1\right\}\right\},\quad \Kbridge  =\left\{\cap_{i=1}^{N-1}\mathcal{K}^{2}_{t_i}\right\}.
  \end{align*} 
% \begin{subequations}\label{eq:new-set}
% \begin{empheq}{align}
%   \hspace*{-2cm}
%     \Kbound&=\left\{\cap_{i=1}^{N-1}\mathcal{K}^{r}_{t_i}\cap \mathcal{K}_{t_0}\cap \mathcal{K}_{t_{N}}|\forall r \in \left\{0,1\right\}\right\},\\
%     \Kbridge  &=\left\{\cap_{i=1}^{N-1}\mathcal{K}^{2}_{t_i}\right\}.
% \end{empheq} 
% \end{subequations}
By following BI (\S.\ref{sec:Bregman-iteration}), we execute optimization w.r.t. (\ref{eq:mmSB-formulation}) while projecting the solution to subset of $\Kbound$ or $\Kbridge$ iteratively. The sketch can be found in Fig.\ref{fig:DMSB_procedure}. The next sections will provide more details on obtaining the joint distribution $\mu$ and optimizing within each constraint set.
\subsection{Optimization in set $\Kbound$}\label{sec:Kbound-opt}
  We first demonstrate how to optimize $\rvz_t^{\theta}$ w.r.t. objective function (\ref{eq:mmSB-formulation}) given the reference path measure $\bar{\pi}^{\phi}$ under one subset of $\Kbound$. The same procedure can be applied to other subsets in $\Kbound$ due to the constructional similarity.
  \begin{proposition}[Optimality w.r.t. $\Kbound$]\label{prop:bound-opt}
    Given the reference path measure $\bar{\pi}^{\phi}$ driven by the policy $\widehat{\rvz}_t^{\phi}$ from boundary $\mu_{t_{i+1}}$ in the reverse time direction, the optimal path measure in the forward time direction of the following problem
    \begin{align*}
      &\min_{\pi} \mathcal{J}(\pi):=\sum_{i=0}^{N-1}KL\left(\pi_{t_i,t_{i+1}}|\bar{\pi}^{\phi}_{t_i,t_{i+1}}\right), \quad s.t \quad \pi &\in \left\{{\int\pi_{t_{i}t_{i+1}}\rd\rvm_{t_{i+1}}=\mu_{t_i}, \int\mu_{t_i}\rd\rvv_{t_i}=\rho_{t_i}}\right\}
    \end{align*}
    \begin{align*}
      \text{is}:\quad \quad \pi_{t_{i}t_{i+1}}^{*}&=\frac{\rho_{t_{i}}\bar{\pi}^{\phi}_{t_i,t_{i+1}}}{\int \bar{\pi}^{\phi}_{t_i,t_{i+1}}\rd\rvm_{t_{i+1}}\rd\rvv_{t_i}}.
    \end{align*}
    When $\pi^{\theta}_{t_{i}t_{i+1}}\equiv \pi^{*}_{t_{i}t_{i+1}},$ 
    % \begin{align*}
    %   \pi^{\theta}_{t_{i}t_{i+1}}\equiv \pi^{*}_{t_{i}t_{i+1}},
    % \end{align*}
    the following equations need to hold $\forall t \in [t_{i},t_{i+1}]$:
    \begin{subequations}
    \begin{align}
        \norm{\rvz_t^{\theta}+\widehat{\rvz}^{\phi}_t-g\nabla_{\rvv}\log p_t^{\phi}}_2^2=0, \label{eq:MM-Kbound}\\
        p_{t_i}(\rvv_{t_i}|\rvx_{t_i})\equiv q^{\phi}_{t_i}(\rvv_{t_i}|\rvx_{t_i}).\label{eq:conditional-generation}
    \end{align}
    \end{subequations}
  \end{proposition}
  Notably, eq.\ref{eq:MM-Kbound} corresponds to the likelihood objective (Prop.\ref{prop:likelihood-obj}). Hence, one can leverage such objective function to optimize $\rvz_t^{\theta}$ after discretizing time:
  \begin{align*}
    \mathcal{L}_{MM}&=\E\left[|| \delta_t\rvz^{\theta}_{t}(\rvm_{t+\delta_t})+\delta_t\widehat{\rvz}^{\phi}_{t+\delta_t}(\rvm_{t+\delta_t}) -\left(\rvm_t+\delta_t \rvz_t^{\theta}-\rvm_{t+\delta_t}\right)||^2\right].
  \end{align*} 
  The velocity boundary condition for the reference path measure in the next BP is encoded in $p_{t_i}(\rvv_{t_i}|\rvx_{t_i}^{\phi})$, but the representation of such conditional distribution is not clear. We leverage the favorable property of SB  to parameterize and sample from such distribution. 
  
  \begin{proposition}[\cite{anderson1982reverse,nelson2020dynamical}]\label{prop:langevin-Law}
    If $\pi^{\theta}$ and $\bar{\pi}^{\phi}$ shares same path measure, then
    \begin{align}
        \tilde{p}_{t_i}^{\theta,\phi}(\rvv_{t_i},\rvx_{t_i}) \equiv q^{\phi}_{t_i}(\rvv_{t_i},\rvx_{t_i})\propto q^{\phi}_{t_i}(\rvv_{t_i}|\rvx_{t_i}),
    \end{align}
    \begin{align}\label{eq:conditional-score}
        \text{where:}\quad \quad \quad \nabla_{\rvv}\log \tilde{p}_t^{\theta,\phi}=\left(\rvz^{\theta}_t+\widehat{\rvz}^{\phi}_t\right)/g.
    \end{align}
  \end{proposition}
  \vskip -0.1in
  Prop.\ref{prop:langevin-Law} suggests that one can use $p_{t_i}(\rvv_{t_i}|\rvx_{t_i}^{\phi}):=\tilde{p}_{t_i}^{\theta,\phi}$ to imply condition (\ref{eq:conditional-generation}) and obtain samples from such distribution by simulating Langevin dynamics using eq.\ref{eq:conditional-score}. Thus, the half-bridge likelihood training (Prop.\ref{eq:half-bridge}) can be applied directly to optimize $\rvz_t^{\theta}$.

  \begin{remark}
    When the ground truth distributions of velocity $\gamma_{t}$ are available, one can simply sample from $\gamma_{t}$ instead of simulating Langevin dynamics.
  \end{remark}
  
  \subsection{Optimization in set $\Kbridge$}\label{sec:kbridge-opt}
  The formulation of optimization under $\Kbridge$ is similar to the previous section:
  \begin{proposition}[Optimality w.r.t. $\Kbridge$]\label{prop:bound-bridge}
    Given the reference path measure $\bar{\pi}^{\phi}$ driven by the policy $\widehat{\rvz}_t^{\phi}$ from boundary $\mu_{t_N}$ in the reverse time direction, the optimal path measure in the forward time direction of the following problem
    \begin{align*}
      \min_{\pi} \mathcal{J}(\pi)&:=\sum_{i=0}^{N-1}KL\left(\pi^{\theta}_{t_i,t_{i+1}}|\bar{\pi}^{\phi}_{t_i,t_{i+1}}\right), \quad s.t \quad \pi \in \Kbridge  =\left\{\cap_{i=1}^{N-1}\mathcal{K}^{2}_{t_i}\right\}
    \end{align*}
    \begin{align*}
      \text{is:}\quad \pi_{t_{0}t_{N}}^{*}&=\frac{q^{\phi}_{t_0}\bar{\pi}^{\phi}_{t_0,t_{N}}}{\int \bar{\pi}^{\phi}_{t_0,t_{N}}\rd\rvm_{t_N}\rd\rvv_{t_0}}.
    \end{align*}
    when $\pi^{\theta}_{t_{0}t_{N}}\equiv \pi^{*}_{t_{0}t_{N}}$,
    % \begin{align*}
    %   \pi^{\theta}_{t_{0}t_{N}}\equiv \pi^{*}_{t_{0}t_{N}}
    % \end{align*}
    the following equations need to hold $\forall t \in [t_{0},t_{N}]$:
    \begin{subequations}
        \begin{align}
            &\norm{\rvz_t^{\theta}+\widehat{\rvz}^{\phi}_t-g\nabla_{\rvv}\log p_t^{\phi}}_2^2=0 \label{eq:MM-Kbound-bridge}\\
            &p_{t_0}(\rvv_{t_0},\rvx_{t_0})\equiv q^{\phi}_{t_0}(\rvv_{t_0},\rvx_{t_0})\label{eq:conditional-generation-bridge}
        \end{align}        
    \end{subequations}
  \end{proposition}
  Conceptually, the above optimization objective with $\Kbridge$ constrain is aiming to find a \emph{continuous} path measure which is close to nominating path measure $\bar{\pi}$ while any intermediate marginals constraints will not be considered. Eq.\ref{eq:MM-Kbound-bridge} can be implied by same objective $\Lmm$ between time range $t\in[t_0,t_N]$. The boundary condition of reference path measure in the next iteration $p_{t_0}(\rvv_{t_0},\rvx_{t_0})$ is determined by eq.\ref{eq:conditional-generation-bridge}. Fortunately, the empirical samples from this distribution are available, though the analytic representation of the distribution $q^{\phi}_{t_0}(\rvv_{t_0},\rvx_{t_0})$ is unknown. Hence we can utilize these samples as empirical sources from boundary distribution $q^{\phi}_{t_0}(\rvv_{t_0},\rvx_{t_0})$ for the next iteration.
  \subsection{Training Scheme}\label{sec:training-scheme}
  Here we introduce the scheme to traverse BI (see Fig.\ref{fig:DMSB_procedure}). In one BI, all constraints must be iterated once. For the sake of $\Lmm$, the reference path measure should be induced by opposite direction. A single BI cannot be recursively repeated due to the conflict of reference path measure direction. For example, at the end of $d$-th BI, $\bar{\pi}$ will be yielded by forward policy while the first BP of $d$-th BI is also optimizing forward policy which violates $\Lmm$ objective. Instead, we reschedule the optimization order. Specifically, in $(d+1)$-th BI, we optimize backward policy at first BP and last BP.

